Local Non-Cooperative Games with Principled Player Selection for Scalable Motion Planning

Game-theoretic motion planners are a powerful tool for the control of interactive multi-agent robot systems. Indeed, contrary to predict-then-plan paradigms, game-theoretic planners do not ignore the interactive nature of the problem, and simultaneously predict the behaviour of other agents while considering change in one's policy. This, however, comes at the expense of computational complexity, especially as the number of agents considered grows. In fact, planning with more than a handful of agents can quickly become intractable, disqualifying game-theoretic planners as possible candidates for large scale planning. In this paper, we propose a planning algorithm enabling the use of game-theoretic planners in robot systems with a large number of agents. Our planner is based on the reality of locality of information and thus deploys local games with a selected subset of agents in a receding horizon fashion to plan collision avoiding trajectories. We propose five different principled schemes for selecting game participants and compare their collision avoidance performance. We observe that the use of Control Barrier Functions for priority ranking is a potent solution to the player selection problem for motion planning.

==> notes.tex <==
constrained Nash equilibrium trajectories in multi-player dynamic game 
(General Nash Equilibrium) deals with
for coupled constrained such as collision avoidance constraints demonstrate the performance through 
previous works with linear quadratic systems iLQG, 

consider a general framework for solving dynamic game
nonlinear constraint and nonlinear cost 


stochastic games that incorporate uncertainty

Algame, david work and how it

safely interact 

interactive traffic scenarios that are challenging for non-game-theoretic trajectory planners
level of interaction between players

predict-then-plan vs the two at the same time is formulated in a game theoretic fashion. (literature)
joint trajectory prediction and planning can be formulated as a dynamic game (literature) 

run online by a 




